Task Grouping for Automated Multi-Task Machine Learning via Task Affinity Prediction

When a number of similar tasks have to be learned simultaneously, multi-task learning (MTL) models can attain significantly higher accuracy than single-task learning (STL) models. However, the advantage of MTL depends on various factors, such as the similarity of the tasks, the sizes of the datasets, and so on; in fact, some tasks might not benefit from MTL and may even incur a loss of accuracy compared to STL. Hence, the question arises: which tasks should be learned together? Domain experts can attempt to group tasks together following intuition, experience, and best practices, but manual grouping can be labor-intensive and far from optimal. In this paper, we propose a novel automated approach for task grouping. First, we study the affinity of tasks for MTL using four benchmark datasets that have been used extensively in the MTL literature, focusing on neural network-based MTL models. We identify inherent task features and STL characteristics that can help us to predict whether a group of tasks should be learned together using MTL or if they should be learned independently using STL. Building on this predictor, we introduce a randomized search algorithm, which employs the predictor to minimize the number of MTL trainings performed during the search for task groups. We demonstrate on the four benchmark datasets that our predictor-driven search approach can find better task groupings than existing baseline approaches.

==> response.tex <==
\clearpage
\nolinenumbers
\setcounter{page}{1}

\pagestyle{plain}
\setlength{\parskip}{\baselineskip}
\setlength{\parindent}{0pt}

\newcounter{reviewercomment}[subsection]
\newcounter{reviewerquestion}[subsection]
\newcommand{\reviewerComment}[1]{\textbf{Comment:} {\it #1}}
\newcommand{\reviewerQuestion}[1]{\textbf{Question:} {\it #1}}
\definecolor{darkblue}{rgb}{0,0,0.5}
\newcommand{\response}[1]{\underline{Response:} {#1} \vspace{0.1in}}
\newcommand{\paperQuote}[1]{``\color{darkblue}\textit{#1}\color{black}''}

\allowdisplaybreaks

\begin{center}
\large{Response to Prior Reviews}\\
\vspace{0.1in}
\centering \large{\textbf{Task Grouping for Automated Multi-Task Machine Learning via Task Affinity Prediction}} \\
\vspace{0.1in}
\large{AAAI-23 Submission \#9603}
\end{center}

This paper was previously submitted to the 37th AAAI Conference on Artificial Intelligence (AAAI-23), under the same title and tracking number \#9603, but it was not accepted for publication. Please find below our responses to the reviews, the version of our paper that was submitted to AAAI-23, and the original reviews.


\subsection*{Reviewer \#6}

\reviewerComment{This work studies the very important question of identifying tasks that should be learned together in multi-task learning.}

\reviewerComment{The Abstract is too long to show the novelty and major contribution of this work.}

\response{We thank the reviewer for their feedback. We have attempted to shorten the abstract of our paper; however, we found that any shorter version lacked some information that we believed to be crucial for the positioning of our work in the literature and for the clear description of our contributions.}

\reviewerComment{For an experiment-driven method, it is not enough to investigate only a small number of datasets (only three sets of tasks, even if there are many tasks) to get the features related to the relationship between tasks. The conclusions drawn from these experiments are not very much convincing and valid.}

\reviewerQuestion{Why only three sets of datasets are considered? Whether the conclusion derived from three datasets only can be valid?}

\response{We agree that evaluation on multiple datasets is crucial for generalization. Recent prior work on task grouping used fewer datasets and tasks than our study: \citeauthor{fifty2021efficiently}~\shortcite{fifty2021efficiently} used two datasets (9 and 5 tasks each), while \citeauthor{standley2020tasks}~\shortcite{standley2020tasks} used only one dataset with two sets of tasks (5 tasks each). 
We believed more datasets to be important and used three benchmark datasets from diverse domains with significantly more tasks (139, 35, \& 29) in our AAAI-23 submission. Despite their differences, we identified common patterns in all three datasets, which suggests that our findings apply more generally.
\emph{Following the reviewer's suggestion, we have included one more dataset (Parkinson's dataset with 42 tasks) in our IJCAI-23 submission.}
}

\reviewerComment{The task-inherent features considered lack good justifications and seem quite arbitrary.}

\newpage
\reviewerQuestion{How can we make sure the features considered are enough for predicting the task affinity?}

\response{We aim to capture similarities between tasks based on various notions of mathematical distances; we studied 68 features in our AAAI-23 submission for capturing task similarity, among which some are motivated by prior work \cite{bingel2017identifying,standley2020tasks}. We identified the most useful features based on correlation and prediction performance (measured using $R^2$), and later considered them for groupwise affinity. 
\emph{In our IJCAI-23 submission, we study two new pairwise-task features}, which we also utilize as groupwise-task features for predicting the task affinity of a group. In general, \emph{the performance of the features for task-affinity prediction can be observed in our experiments: they explained 43\%, 94\%, 21\%, and 36\% of the variance in task affinity} in the School, Chemical, Landmine, and Parkinson's datasets, respectively (\cref{fig:predictor_groupwise}).}


\reviewerComment{The organisation of the paper is not easy to follow. The paper starts with an experimental investigation at the very beginning of the paper without a clear description of the problem even. There are many sets of experiments in different sections but there is also a specific section for numerical results.}

\response{We thank the reviewer for pointing out that the organization of our paper needs more explanation.
Our paper begins in the usual manner by providing context and motivation for our work and introducing our research problem (\cref{sec:intro}), followed by an overview of the state of the art (\cref{sec:related}).
Then, we describe the four benchmark datasets and our experimental setup (\cref{sec:experiment_setup}). 
The rationale behind describing these near the beginning of our paper is that we utilize these benchmark datasets repeatedly throughout the paper, studying pairwise affinity, groupwise affinity, and algorithms for task grouping.
Next, we study pairwise affinity and introduce features that can capture the relationship between two tasks from the perspective of MTL (\cref{subsec:pairwise_affinity}).
We include numerical results pertaining to this topic in \cref{subsec:pairwise_affinity} (instead of including them in a dedicated section on numerical results) because general conclusions drawn from these results are crucial part of our study, and we wanted to save the reader from having to go back-and-forth between \cref{subsec:pairwise_affinity} and a dedicated section on numerical results.
Similarly, we present our study of groupwise affinity with numerical results included in \cref{subsec:group_affinity} since these results are crucial part of the study.
Based on the findings of the task-affinity studies, we propose a randomized local search for task grouping that incorporate a task-affinity predictor to improve search performance (\cref{sec:approach}).
Finally, we present numerical results on our proposed search approach, comparing it with existing approaches from the state of the art, demonstrating significant improvement (\cref{sec:result}).
We have revised our paper to explain its organization better (e.g., we added an explanation to the beginning of \cref{sec:experiment_setup}.)}


\subsection*{Reviewer \#7}

\reviewerComment{The paper was reasonably clearly written and the results are convincing in the small data domain that the authors selected.}

\reviewerComment{However, it would have been more convincing had the authors also applied the method to the data used in Fifty et al.\ (2021) and Standley et al.\ (2020). First, the datasets are much bigger.}

\reviewerComment{Second, the datasets there are not featurized in the way that datasets from the UCI machine learning datasets would be, but are rather `featurized' by the NN architecture itself and there's no evidence that this method would work on images or text which utilize such architectures.}

\response{We did not use datasets from the studies of \citeauthor{fifty2021efficiently}~\shortcite{fifty2021efficiently} (two datasets with 9 and 5 tasks) or \citeauthor{standley2020tasks}~\shortcite{standley2020tasks} (one dataset with two sets of 5 tasks each) since they consist of \emph{significantly fewer tasks} than our benchmarks datasets (e.g., 139 tasks in one of the datasets). With only a few tasks, an exhaustive search is feasible. \citeauthor{standley2020tasks}~\shortcite{standley2020tasks} indeed perform an exhaustive search for task grouping (only $2^5-1=31$ possible groups). 
This approach is clearly infeasible for datasets that include large numbers of tasks (see paragraph \emph{Exhaustive Search} in \cref{sec:baseline_approaches}).
\emph{Our paper focuses on this problem setting: how to predict task affinity and find optimal groups of tasks for MTL in a dataset that consists of a large number of tasks?}
We study these questions using four widely-used MTL datasets \cite{zhang2021survey} and show that our approach significantly improves over the state of the art (\cref{sec:result}).}

\reviewerQuestion{`number of samples are good predictors of group affinity'? Just seems to be a coincidence. Can you provide more evidence than just the examples here? Being able to draw a similar conclusion from a much larger swathe of tasks and datasets would be more convincing.}

\response{We agree that general conclusions are more convincing when they are based on multiple datasets.
Recent prior work on task grouping used fewer datasets and tasks than our study: \citeauthor{fifty2021efficiently}~\shortcite{fifty2021efficiently} used two datasets (9 and 5 tasks each), while \citeauthor{standley2020tasks}~\shortcite{standley2020tasks} used only one dataset with two sets of tasks (5 tasks each). 
We believed more datasets to be important and used three benchmark datasets from diverse domains with significantly more tasks (139, 35, \& 29) in our AAAI-23 submission. Despite their differences, we identified common patterns in all three datasets, which suggests that our findings apply more generally.
\emph{Following the reviewer's suggestion, we have included one more dataset (Parkinson's dataset with 42 tasks) in our IJCAI-23~\mbox{submission.}}%
}

\newpage
\subsection*{Reviewer \#8}

\reviewerComment{Strengths: (1) The motivation of this paper is interesting, which aims to deal with the problem of inter-task interference by task grouping.
(2) This paper proposed a task-grouping strategy with a predictor to accelerate the re-grouping and evaluating process.}

\reviewerComment{The section ``Study of Task Affinity" provides too straightforward and task-specific findings. For example, ``the useful features for prediction also have a high correlation with the relative MTL gain,'' which is meaningless and should not be claimed as a finding.}


\response{By studying four different benchmark datasets (three in our original AAAI-23 submission) from diverse domains \cite{zhang2021survey}, we aim to provide results from which we can draw general conclusions.
For example, we find that features based on the single-task learning-curve gradients%
, the variance and standard deviation of the target attribute of each task, and the difference in the sample sizes of the tasks are useful for predicting relative pairwise MTL gain across multiple benchmark datasets. 
We also find that the average pairwise MTL gain and the average dot product of task-specific parameters are good predictors of groupwise affinity across all benchmark datasets.
\emph{Such general conclusions from our task-affinity study are not dataset specific, and they are useful for finding groups of tasks for MTL} (e.g., with our proposed randomized local search), which in turn can reduce MTL losses.
\emph{To strengthen our results, we have included one more dataset in our IJCAI-23 submission, in addition to the three datasets of our AAAI-23 submission.} With respect to the relation between feature usefulness and correlation, we would like to highlight that while correlation does imply usefulness, vice versa is not necessarily true.}

\reviewerComment{The experiments are too simple where the baseline is only ``Randomized Search Baseline.'' Where are the results of STL, standard MTL, and other SOTA MTL methods?}


\response{We apologize for not making the goal of our work clear enough. Our goal is orthogonal to the performance of specific MTL methods; we are interested in predicting which tasks will benefit from MTL and finding groups of tasks that should be learned together using MTL. 
In fact, \emph{our search approach can potentially benefit a wide range of MTL methods by identifying tasks that should be learned together}. 
Therefore, we must compare our proposed search approach to existing approaches for grouping tasks together for MTL.
In our IJCAI-23 submission, \emph{we provide a comparison to recent, state-of-the-art work in this area}~\cite{fifty2021efficiently,standley2020tasks,bingel2017identifying}, demonstrating the advantage of proposed search approach.
Further, we also compare our approach to STL, simple variations of SOTA MTL, etc.
We report the most important results in \cref{tab:comparison_with_SOTA_MTL} and all remaining results in \cref{tab:clustering_results} in \cref{appendix:extra_results}.
}




\newpage
\reviewerComment{Missing baselines. To deal with task interference, many other works proposed strategies like dynamic weighting, Pareto MTL, or just designing some useful networks [1-3].
References:\newline
[1] Xiao L, Zhang H, Chen W. ``Gated multi-task network for text classification. NAACL, 2018, 726-731.\newline
[2] Lin X, Zhen H L, Li Z, et al. ``Pareto multi-task learning.'' Advances in Neural Information Processing Systems, 2019, 32.\newline
[3] Fifty, Chris, et al. ``Efficiently identifying task groupings for multi-task learning.'' Advances in Neural Information Processing Systems 34 (2021), 27503-27516.
}

\response{
The method proposed by \citeauthor{fifty2021efficiently}~\shortcite{fifty2021efficiently} (Ref. 3) is the closest to our work. However, their approach applies to significantly smaller settings, requiring training one extensive network with all tasks and explicitly measuring pairwise affinity between them. In contrast, we present a scalable pairwise-affinity predictor, which uses features that can be computed easily. In our IJCAI-23 submission, we have applied the \textit{inter-task affinity} calculation method proposed in \cite{fifty2021efficiently}, and we compared these \emph{inter-task affinity} values with actual pairwise affinities (measured as relative MTL gain) after training multi-task learning models for each pair. 
According to our empirical results, even though the \emph{inter-task affinity} values correlate with actual pairwise affinities, they are not a particularly strong predictor in comparison with other, simpler features.
Further, the grouping search used by \cite{fifty2021efficiently} is a simple exhaustive search, which would be infeasible in our setting (9 tasks in their setting vs. 139 tasks in ours). We propose a novel groupwise-affinity predictor to implement a more efficient guided search.
Prior work by \citeauthor{xiao2018gated}~\shortcite{xiao2018gated} (Ref. 1) is very specific to CNNs, while \citeauthor{lin2019pareto}~\shortcite{lin2019pareto} (Ref. 2) do not address the problem of task grouping.
}

\reviewerComment{How to guarantee the multi-task optima (Pareto solutions)? Is it possible that the task-group predictor does not work in more general datasets?}

\response{In this paper, we run our randomized search approach with the objective of minimizing loss over all tasks. However, it would be straightforward to replace the objective function of our search approach with one that considers both loss and, e.g., model complexity measured using number of parameters. Our task-affinity predictor would be able to provide estimates for the loss, which could then be easily combined with, e.g., the number of model parameters to obtain an estimate of the objective function for a new mutation. This straightforward extension could be used to find partitions that minimize both loss and model complexity. 
To ensure that the group-affinity predictor works on `\emph{more general datasets,}' we utilize four different benchmark datasets in our study (three in our original AAAI-23 submission) from diverse domains \cite{zhang2021survey}. 
Across these different datasets, we can easily explain 43\%, 94\%, 21\%, and 36\% of the variance in affinity on the School, Chemical, Landmine, and Parkinson's datasets, respectively (\cref{fig:predictor_groupwise}).}


\newpage
\subsection*{Reviewer \#9}

\reviewerComment{Strengths:
1. This work provides a systematic solution for task clustering when MTL is desirable and feasible.
2. The confirmation that there exist task-relational features with prediction power is valuable.
3. The experiments support the discovery by showing how relative MTL gain can be predicted and impact learning over different datasets.}

\reviewerComment{This method requires the same target across different tasks, therefore not directly applicable to tasks with different goals.}

\response{We thank the reviewer for bringing up this point of discussion. In our study, we consider four widely-used MTL datasets \cite{zhang2021survey} as benchmarks. Each one of these four datasets does indeed consist of a set of tasks that all have the same target attribute. However, \emph{our proposed predictor and search approach do not make such an assumption}; hence, they do not actually rely on all the tasks having the same target.}

\reviewerQuestion{Maybe I missed it, what is the baseline performance if MTL is conducted simply over all the tasks?}

\response{We apologize for not presenting this clearly enough in our AAAI-23 submission.
In our ICJAI-23 submission, we include this result in \cref{tab:comparison_with_SOTA_MTL} (column \textbf{Simple MTL}) in the main text. Our proposed approach very clearly outperforms this baseline.}

\reviewerQuestion{Group mutation (MutateGroups) is entirely random. Any chance a greedy searching method, perhaps considering task-relation, can suggest candidate task replacement even better?}

\response{While the mutation operation \textbf{MutateGroups} (\cref{alg:mutation}) by itself is indeed uniformly random, we integrate it with a \emph{quick reject based on predicted MTL loss}, which is based on our task-affinity predictor (see paragraph \emph{Randomized Local Search with Affinity Predictor} in \cref{subsec:quick_reject}). 
Mutation and quick reject together can be viewed as a `guided mutation' that recommends new partitions which are expected to perform better: since mutations that are predicted to perform poorly are likely to be quickly rejected, the mutations that are actually considered by the search are likely to improve MTL loss.}



